Temporal Linear Item-Item Model for Sequential Recommendation

In sequential recommendation (SR), neural models have been actively explored due to their remarkable performance, but they suffer from inefficiency inherent to their complexity. On the other hand, linear SR models exhibit high efficiency and achieve competitive or superior accuracy compared to neural models. However, they solely deal with the sequential order of items (i.e., sequential information) and overlook the actual timestamp (i.e., temporal information). It is limited to effectively capturing various user preference drifts over time. To address this issue, we propose a novel linear SR model, named TemporAl LinEar item-item model (TALE), incorporating temporal information while preserving training/inference efficiency, with three key components. (i) Single-target augmentation concentrates on a single target item, enabling us to learn the temporal correlation for the target item. (ii) Time interval-aware weighting utilizes the actual timestamp to discern the item correlation depending on time intervals. (iii) Trend-aware normalization reflects the dynamic shift of item popularity over time. Our empirical studies show that TALE outperforms ten competing SR models by up to 18.71% gains on five benchmark datasets. It also exhibits remarkable effectiveness in evaluating long-tail items by up to 30.45% gains. The source code is available at https://github.com/psm1206/TALE.

==> Fig_tex/Fig1.tex <==
\begin{figure}
\begin{tabular}{cc}
\includegraphics[height=3.05cm]{Figures/heat_toys.png} &
\includegraphics[height=3.05cm]{Figures/heat_beauty.png} \\
\multicolumn{1}{c}{(a) ML-1M} &\multicolumn{1}{c}{(b) Beauty}
% \vspace{-2mm}
\end{tabular}

\vspace{1mm}

\begin{tabular}{cc}
\includegraphics[height=3.05cm]{Figures/heat_sports.png} &
\includegraphics[height=3.05cm]{Figures/heat_yelp.png} \\
\multicolumn{1}{c}{(c) Sports} &\multicolumn{1}{c}{(d) Yelp}
\vspace{-2mm}
\end{tabular}
\caption{Item-hop according to time interval.}\label{fig:co-cocurrence}
\vspace{-3mm}
\end{figure}


==> Fig_tex/heat_map_B.tex <==
\begin{figure}
\begin{tabular}{cc}
\includegraphics[height=3.0cm]{Appendix/heat_wo_norm.png} &
\includegraphics[height=3.0cm]{Appendix/heat_w_norm.png} \\
\multicolumn{1}{c}{(a) W/O TN } &\multicolumn{1}{c}{(b) W TN} \\
\end{tabular}

\vspace{2mm}
\caption{Visualization of TALE's weight matrix B (a) without Trend-aware Normalization and (b) with Trend-aware Normalization, on beauty dataset. }\label{fig:heat_map}

\vspace{-2mm}
\end{figure}

==> Fig_tex/hyper_sensi_tau.tex <==
\begin{figure}
\begin{tabular}{cc}
\includegraphics[height=3.0cm]{Figures/hyper_sensitivity/ml-1m_tau.eps} &
\includegraphics[height=3.0cm]{Figures/hyper_sensitivity/beauty_tau.eps} \\
\multicolumn{1}{c}{(a) ML-1M} &\multicolumn{1}{c}{(b) Beauty} \\
\end{tabular}
\vspace{-3mm}
\caption{Performance of TALE over $\tau_{\text{time}}$ for time interval-aware weighting on ML-1M and Beauty.}\label{fig:hyper_tau}

\vspace{-2mm}
\end{figure}

==> Fig_tex/hyper_sensi_window.tex <==
\begin{figure}
\begin{tabular}{cc}
\includegraphics[height=3.0cm]{Figures/hyper_sensitivity/ml-1m_window.eps} &
\includegraphics[height=3.0cm]{Figures/hyper_sensitivity/beauty_window.eps} \\
\multicolumn{1}{c}{(a) ML-1M} &\multicolumn{1}{c}{(b) Beauty} \\
\end{tabular}
\vspace{-3mm}
\caption{Performance of TALE over window size $N$ for trend-aware normalization on ML-1M and Beauty.}\label{fig:hyper_window}

\vspace{-3mm}
\end{figure}

==> Fig_tex/intv_co_occur_appen.tex <==
\begin{figure}
\begin{tabular}{cc}
\includegraphics[height=3.0cm]{Figures/intv_co_occur/AR_sports.png} &
\includegraphics[height=3.0cm]{Figures/intv_co_occur/AR_toys.png} \\
\multicolumn{1}{c}{(a) Toys} &\multicolumn{1}{c}{(b) Sports} 
\end{tabular}

\vspace{1mm}

\begin{tabular}{c}
\includegraphics[height=3.0cm]{Figures/intv_co_occur/AR_yelp.png} \\
\multicolumn{1}{c}{(c) Yelp}
\end{tabular}

\vspace{-2mm}
\caption{Co-occurrences between consecutive items according to time interval on Toys, Sports, and Yelp.  }\label{fig:intv_co_occur_appen}
\vspace{-3mm}
\end{figure}


==> Fig_tex/intv_distribution.tex <==
\begin{figure}
\includegraphics[height=4.5cm]{Figures/distribution.png} 

\caption{Ratio distributions for consecutive items according to time interval on ML-1M, Beauty, Sports, Toys, and Yelp.}\label{fig:intv_distribution}
\end{figure}


==> Fig_tex/intv_perform.tex <==
\begin{figure}
\begin{tabular}{cc}
\includegraphics[height=3.05cm]{Figures/intv_performance/ml_intv_perf.png} &
\includegraphics[height=3.05cm]{Figures/intv_performance/beauty_intv_perf.png} \\
\multicolumn{1}{c}{(a) ML-1M} &\multicolumn{1}{c}{(b) Beauty}
% \vspace{-2mm}
\end{tabular}

\vspace{1mm}

\begin{tabular}{cc}
\includegraphics[height=3.05cm]{Figures/intv_performance/sports_intv_perf.png} &
\includegraphics[height=3.05cm]{Figures/intv_performance/toys_intv_perf.png} \\
\multicolumn{1}{c}{(c) Sports} &\multicolumn{1}{c}{(d) Yelp}
\vspace{-2mm}
\end{tabular}
\caption{Performance comparison between SLIT w/ and w/o temporal information by groups of time interval.}\label{fig:intv_perform}
\vspace{-3mm}
\end{figure}


==> Tables/tab-ablation_perform_.tex <==
\begin{table} \small
\caption{Ablation study of TALE on ML-1M and Beauty. TALE consists of three parts: (1) time interval-aware weighting, (2) trend-aware normalization, and (3) single-target augmentation. Each metric is NDCG@5.}
\label{tab:ablation_performance}
\vspace{-2mm}
\begin{center}
\renewcommand{\arraystretch}{1} % 테이블 행 간격
\begin{tabular}{P{1.1cm}|P{0.7cm}P{0.7cm}P{1.0cm}|P{0.7cm}P{0.7cm}P{1.0cm}}
% \begin{tabular}{c|cc|cc|cc}
\toprule
Dataset         & \multicolumn{3}{c|}{ML-1M}          & \multicolumn{3}{c}{Beauty}              \\
Model              & N@5   & Tail & Head  & N@5   & Tail & Head \\
\midrule
TALE               & \textbf{0.1276} & \textbf{0.0814} & \textbf{0.0277}   & \textbf{0.0482}   & \textbf{0.0271} & \textbf{0.0125}     \\
- (1)              & 0.1227  & 0.0739 & 0.0254 & 0.0450  & 0.0239 & 0.0108     \\
- (2)              & \underline{0.1257}  & \underline{0.0773} & \underline{0.0264} & \underline{0.0468}  & \underline{0.0243} & 0.0111       \\
- (3)              & 0.0473  & 0.0161 & 0.0057 & 0.0296  & 0.0154 & 0.0068    \\
% \midrule
- (1, 2)              & 0.1172  & 0.0685 & 0.0238 & 0.0444 & 0.0235  & 0.0107    \\
- (1, 3)              & 0.1187  & 0.0659 & 0.0230 & 0.0431  & 0.0242  & \underline{0.0112} \\
- (2, 3)              & 0.0430  & 0.0114 & 0.0042 & 0.0303  & 0.0150  & 0.0065 \\
- (1, 2, 3)           & 0.1164  & 0.0624 & 0.0220 & 0.0435  & 0.0235  & 0.0108 \\
% \midrule
% + (4)             & 0.1176  & 0.0781 & 0.0266 & 0.0443 & 0.0271  & 0.0122  \\
% + (1, 4)          & 0.xxxx  & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx  & 0.xxxx  \\
% + (3, 4)          & 0.xxxx  & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx  & 0.xxxx  \\
% + (1, 3, 4)       & 0.xxxx  & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx  & 0.xxxx  \\


\bottomrule
\end{tabular}
% \vspace{-4mm}
\end{center}
\end{table}

==> Tables/tab-hyper_sensitivity.tex <==
\begin{table} % \small
\caption{Ablation study of TALE on ML-1M, Beauty, and Yelp. TALE consists of three components: (1) temporal weighting, (2) trend-aware normalization, and (3) single-target augmentation. The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}. SLIT$_{st}$ denotes SLIT w/ a single target item.}
\label{tab:ablation_performance}
\begin{center}
\renewcommand{\arraystretch}{1} % 테이블 행 간격
\begin{tabular}{P{1.2cm}|P{0.8cm}P{0.8cm}|P{0.8cm}P{0.8cm}}
% \begin{tabular}{c|cc|cc|cc}
\toprule
Dataset         & \multicolumn{2}{c|}{ML-1M}          & \multicolumn{2}{c|}{Beauty}        \\
Model              & H@10      & N@10      & H@10      & N@10      \\
\midrule
0                 & 0.2495    & 0.1474    & 0.0797    & 0.0499    \\
0.2               & 0.2546    & 0.1498    & 0.0588    & 0.0344    \\
0.4               & 0.2427    & 0.1435    & 0.0793    & 0.0501    \\
0.6               & 0.2285    & 0.1370    & 0.0831    & 0.0514    \\
0.8               & 0.2253    & 0.1335    & 0.0594    & 0.0352    \\
1                 & 0.2184    & 0.1284    & 0.0885    & 0.0550    \\


\bottomrule
\end{tabular}
% \vspace{-4mm}
\end{center}
\end{table}

==> Tables/tab-slit1target.tex <==
\begin{table}
\caption{Performance comparison between SLIT and SLIT w/ a single target item (\ie, SLIT$_{st}$).}
\vspace{-1mm}
\label{tab:slit_slit1target}
\begin{center}
\renewcommand{\arraystretch}{1} % 테이블 행 간격
\begin{tabular}{P{1.5cm}|P{1.5cm}|P{1.1cm}P{1.1cm}P{1.1cm}}

\toprule
Dataset   & Model      & N@1         & N@5         & N@10        \\
\midrule
\multirow{2}{*}{ML-1M}
 & SLIT        & 0.0596          & 0.1164          & 0.1377          \\
 & SLIT$_{st}$ & \textbf{0.0609} & \textbf{0.1172} & \textbf{0.1386} \\
\midrule
\multirow{2}{*}{Beauty}
 & SLIT        & \textbf{0.0267}   & 0.0435          & 0.0499          \\
 & SLIT$_{st}$ & 0.0265 & \textbf{0.0440} & \textbf{0.0514} \\
\midrule
\multirow{2}{*}{Sports}
 & SLIT        & 0.0155          & 0.0271          & 0.0315          \\
 & SLIT$_{st}$ & \textbf{0.0169} & \textbf{0.0286} & \textbf{0.0329} \\
\midrule
\multirow{2}{*}{Toys}
 & SLIT        & 0.0333          & 0.0535          & 0.0599          \\
 & SLIT$_{st}$ & \textbf{0.0342} & \textbf{0.0554} & \textbf{0.0621} \\ 
\bottomrule
\end{tabular}
% \vspace{-2mm}

\end{center}
\end{table}


==> Tables/tab-time_correlation.tex <==
\begin{table} % \small
\caption{Pearson correlation coefficients for SLIST and TALE on five datasets.}
\label{tab:time_pearson}
\vspace{-2mm}
\begin{center}
\renewcommand{\arraystretch}{1} % 테이블 행 간격
% \begin{tabular}{P{1.2cm}|P{0.8cm}P{0.8cm}|P{0.8cm}P{0.8cm}}
\begin{tabular}{c|ccccc}
\toprule
Model    & ML-1M   & Beauty   & Toys   & Sports   & Yelp               \\
\midrule
SLIST ~\cite{ChoiKLSL21}& 0.0130 & 0.0524 & 0.0718 & 0.0325 & 0.0910 \\
TALE                 & \textbf{0.0375} & \textbf{0.3944} & \textbf{0.5602} & \textbf{0.5027} & \textbf{0.3885} \\

\bottomrule
\end{tabular}
\end{center}
\end{table}

==> Tables/tab-time_interval_perform.tex <==
\begin{table} % \small
\caption{Accuracy comparison by groups of time interval on ML-1M and Beauty. Each metric is NDCG@5. }
\label{tab:ablation_time_intv_perf}
\vspace{-2mm}
\begin{center}
\renewcommand{\arraystretch}{1} % 테이블 행 간격
\begin{tabular}{P{1.2cm}|P{1.9cm}|P{0.9cm}P{0.9cm}P{0.9cm}}
% \begin{tabular}{c|cc|cc|cc}
\toprule
Dataset & Model    & Short & Mid  & Long  \\
\midrule
\multirow{4}{*}{ML-1M} 
& BSARec~\cite{ShinCWP24}         & \textbf{0.2124}    & 0.1233    & 0.0310 \\
& TiSASRec~\cite{LiWM20}          & 0.2025    & 0.1202    & 0.0312  \\
& SLIST~\cite{ChoiKLSL21}       & 0.1593    & 0.1497    & 0.0402 \\
& TALE                          & 0.1780    & \textbf{0.1584}    & \textbf{0.0465} \\
\midrule
\multirow{4}{*}{Beauty} 
& BSARec~\cite{ShinCWP24}         & 0.0506    & 0.0424    & 0.0078 \\
& TiSASRec~\cite{LiWM20}          & 0.0483    & 0.0458    & 0.0077 \\
& SLIST~\cite{ChoiKLSL21}        & 0.0621    & 0.0532    & 0.0110 \\
& TALE                          & \textbf{0.0755}    & \textbf{0.0560}    & \textbf{0.0115} \\
\bottomrule
\end{tabular}
% \vspace{-4mm}
\end{center}
\end{table}

==> Tables/tab-time_interval_statistics.tex <==
\begin{table}[t]
\begin{center}
\caption{Time-interval statistics of five benchmark sequential datasets. The time unit is day.}
\vspace{-2mm}
\label{tab:time_interval_statistics}
\begin{tabular}{c|cccccc}
\toprule
Dataset & ML-1M & Beauty & Toys & Sports & Yelp & KuaiRand \\
\midrule
Mean & 165.6 & 8.9 & 8.6 & 8.3 & 10.4 & xx.x \\
Std. & 165.6 & 8.9 & 8.6 & 8.3 & 10.4 & xx.x \\
\bottomrule
\end{tabular}

\end{center}
\vspace{-3mm}
\end{table}

